Observations of the Optical Afterglow of GRB 050319 : Wind to ISM transition in view

The collapse of a massive star is believed to be the most probable progenitor of a long GRB. Such a star is expected to modify its environment by stellar wind. The effect of such a circum-stellar wind medium is expected to be seen in the evolution of a GRB afterglow, but has so far not been conclusively found. We claim that a signature of wind to constant density medium transition of circum-burst medium is visible in the afterglow of GRB 050319. Along with the optical observations of the afterglow of GRB 050319 we present a model for the multiband afterglow of GRB 050319. We show that the break seen in optical light curve at $\sim$ 0.02 day could be explained as being due to wind to constant density medium transition of circum-burst medium, in which case, to our knowledge, this could be the first ever detection of such a transition at any given frequency band. Detection of such a transition could also serve as a confirmation of massive star collapse scenario for GRB progenitors, independent of supernova signatures.

==> readme <==
%auto-ignore

This file contain information regarding the paper 
"Observations of the Optical Afterglow of GRB 050319 : Wind to ISM transition in view "

Authors: Atish Kamble, L. Resmi, Kuntal Misra 

The contact details of the first author are as follows

email  : atish@rri.res.in
	 atish.vyas@gmail.com	

Comments:  11 pages, 3 tables, 1 figures. Published in ApJ Letters. 
The definitive version is available at http://www.journals.uchicago.edu/

Abstract:
The collapse of a massive star is believed to be the most probable progenitor
of a long GRB. Such a star is expected to modify its environment by stellar wind.
The effect of such a circum-stellar wind medium is expected to be seen
in the evolution of a GRB afterglow, but has so far not been conclusively found.
We claim that a signature of wind to constant density medium transition
of circum-burst medium is visible in the afterglow of GRB 050319.
Along with the optical observations of the afterglow of GRB 050319
we present a model for the multiband afterglow of GRB 050319. We show that
the break seen in optical light curve at $\sim$ 0.02 day could be explained
as being due to wind to constant density medium transition of circum-burst medium,
in which case, to our knowledge, this could be the first ever detection of such
a transition at any given frequency band. Detection of such a transition
could also serve as a confirmation of massive star collapse scenario
for GRB progenitors, independent of supernova signatures.

 The compressed tar file "GRB050319.tar.gz" contain the following files:
 readme                 This file
 aastex.cls          	LaTeX class file
 apj.bst		LaTeX class file
 ms.tex                 LaTeX file of the paper
 fig1.ps                Figure 1 in the paper

